Discovering Domain Orders through Order Dependencies

Much real-world data come with explicitly defined domain orders; e.g., lexicographic order for strings, numeric for integers, and chronological for time. Our goal is to discover implicit domain orders that we do not already know; for instance, that the order of months in the Chinese Lunar calendar is Corner < Apricot < Peach. To do so, we enhance data profiling methods by discovering implicit domain orders in data through order dependencies. We enumerate tractable special cases and proceed towards the most general case, which we prove is NP-complete. We show that the general case nevertheless can be effectively handled by a SAT solver. We also devise an interestingness measure to rank the discovered implicit domain orders, which we validate with a user study. Based on an extensive suite of experiments with real-world data, we establish the efficacy of our algorithms, and the utility of the domain orders discovered by demonstrating significant added value in three applications (data profiling, query optimization, and data mining).

==> approximate.tex <==
\begin{change}
\section{Approximate Order Compatibilities}
When considering approximated order compatibilities, one natural approach is to define approximate SOCs given some parameter $\alpha$, as SOCs that hold if we remove at most ratio $\alpha$ of the tuples from the database. For \emph{SynOC}s, this definition can be implemented in the same way as regular OCs, which can be done in leaner time and has been discussed in \cite{FOD}. We will now discuss extending this idea to $SemOC_{sc}$'s and $SemOC_{gc}$'s and their respective difficulties in more details.
\todo{is the syntactic version the same as the OD one?}

\subsection{Approximate $SemOC_{sc}$}
Despite the validation of $SemOC_{sc}$'s having an efficient polynomial algorithm, trying to find the minimum number of rows that are necessary to make a $SemOC_{sc}$ valid would introduce NP-hardness to the problem. This problem occurs when merging partial order graphs derived from multiple contexts. The NP-hardness of this problem could be proved using a reduction from the \emph{minimum feedback arc set} (MFAS) problem which is the problem of finding the minimum number of edges in a directed graph whose removal would make the graph acyclic and has been shown to be NP-hard\cite{GareyJohnsonBook}.

\begin{lemma} (Approximate $SemOC_{sc}$ with minimum tuple removal is NP-hard)
The problem of finding the minimum number of tuples whose removal would make a $SemOC_{sc}$ candidate valid is NP-hard.
\end{lemma}

\textbf{Proof Sketch:} Consider an instance of the MFAS problem, which is a directed graph. For each edge $(u, v)$ in the graph, construct a new context with only two tuples $(1, u)$ and $(2, v)$. These tuples would induce the order $u\le v$ in this context and would be considered when merging multiple partial orders from different contexts together. Finding the minimum number of tuples in this database whose removal would make the candidate a valid $SemOC_{sc}$ is equivalent to finding the solution to the MFAS problem, which shows the original problem to be NP-hard. 


\subsection{Approximate $SemOC_{gc}$}
The main difficulty with using the idea of row removal for $SemOC_{gc}$'s is the difficulty when merging partial orders from multiple contexts. Despite the NP-completeness of the decision problem in validating $SemOC_{gc}$'s, since finding even only two polarity groups that were impossible to merge was enough to invalidate a candidate, practical cases were usually solved in a short time. However, aiming to find the minimum number of tuples that would fix (potentially multiple) inconsistent polarity groups could be much harder to achieve, despite the comparative tractability of the decision problem in practice.
\end{change}

% \subsection{Approximate \emph{SynOC}}
% Assuming we are going with the minimal repair principle and looking for a dependency that holds with the minimum number of tuple having to be removed:
% \\ Let’s consider the order compatibility candidate $A \sim B$ with the error threshold alpha (if is 0.05, we can afford to remove up to \%5 of the tuples for the dependency to hold.)
% \begin{algorithm}[h]
%   \begin{small}
%     \caption{apprSynOC} \label{pc:apprSynOC}
%     \begin{algorithmic}[1]
%         \FOR{each two sequential equivalence classes in A (Ai and Ai+1)}
%             \STATE index = 0
%             \STATE Find corresponding equivalence classes in B whose tIDs fall in Ai (call it bCurrList) and in Ai+1(call it bNextList)
%             \STATE currMax  = value for last equivalence class in bCurrList
%             \STATE nextMin = value for bNextList[index]
%             \WHILE{$(nextMin < currMax) and (error < )$}
%                 \STATE $error += |bNextList[index]| / t$  % t is the number of tuples
%                 \STATE $index += 1$
%             \ENDWHILE
%             \IF{$error > alpha$}
%                 \RETURN 0
%             \ENDIF
%             \STATE print (``approximate dependency found'')
%         \ENDFOR
%     \end{algorithmic}
%   \end{small}
% \end{algorithm}


% \\ Basically, if there is a swap, we add the size of the first equivalence class in the sorted partition of B (corresponding to the tuples that fall in the next equivalence class of sorted partition on A) to our error variable and move on to the next smallest equivalence class until we reach an equivalence class that is equal to or bigger than the largest equivalence class from the previous list, that means we’ve disregarded enough tuples for the swaps to go away and we can move on to the next equivalence classes in sorted partition on A.
% Complexity for this seems to be linear. seems to be as expensive as validating an absolute OC.

% % \begin{colorful}
% % \subsection{Approximate $SemOC_{gc}$}

% % The initial approach we had in mind of finding approximate $SemOC_{gc}$s, was to create the elements graph and remove edges so that the remaining graph would be cycle free and less than $\alpha$ fraction of the tuples would have to be removed in the process.

% % %%% checked till here

% % There are a couple of issues with this approach:
% % \begin{enumerate}
% %     \item When an individual equivalence class produces an invalid bipartite graph invalid, how would one even derive a chain out of it to add it to the elements graph? Take Table \ref{tab:approxGenSOC} and its corresponding bipartite graph in Figure \ref{fig:approxGenSOC} for example:
% %     %% find the graph that's being talked about in the paragraph above
% %     \begin{table}[H]
% %     \centering
% %     \caption{\label{tab:approxGenSOC}}
% %     \begin{tabular}{|c|c|}
% %     \hline
% %         $\A{A}$ & $\A{B}$  \\
% %         \hline
% %          \hline
% %          a & 1  \\
% %          \hline
% %          c & 1  \\
% %          \hline
% %          c & 3  \\
% %          \hline
% %          c & 2  \\
% %          \hline
% %          d & 3  \\
% %          \hline
% %          b & 2  \\
% %     \hline
% %     \end{tabular}
% % \end{table}
    
% % \begin{figure}[!ht]
% %     \center{\includegraphics[width=3cm]
% %     {figs/approxGenSOC1.png}}
% %     \caption{\label{fig:approxGenSOC} biGraph corresponding to Table \ref{tab:approxGenSOC}}
% % \end{figure}
    
% %     \\
% %     If we were to derive one chain out of this graph, it would either have to be [a, c, d] or [a, c, b] or [b, c, d]. One thing we could do in this case, is to produce all possible chains and pass those on to be added to the elements graph. This would translate to the addition of the chains in Figure \ref{fig:approxGenSOC2} to the elements graph.
    
% % \begin{figure}[!ht]
% %     \center{\includegraphics[width=7cm]
% %     {figs/approxGenSOC2.png}}
% %     \caption{\label{fig:approxGenSOC2} individually valid partial orders derived from Figure \ref{fig:approxGenSOC}}
% % \end{figure}
% %     The number of such chains could grow larger depending on the number of nodes with a branch-out and the number of their non-singleton branches.
% %     Out of all these chains, only one of them should remain in the final elements graph. Therefore, if we incorporate all these chains in the elements graph, how do we enforce that only one version remains in the end while also removing enough edges to make the graph cycle-free?
% %     \\
    
% %     \item Even if the issue above is resolved, when we say we should remove an edge from the elements graph, what would that translate into in terms of tuples in the table? Each edge in the elements graph is created by at least 2 tuples in the table. (e.g. edge $a \rightarrow c$ is created by tuples (a, 1) and (c, 1) in the table above.  Same edge might also have been made from (a, 2) and (c, 2) from another equivalence class. Which of these four edges have to be removed if it is determined that $a \rightarrow c$ needs to be cut from the elements graph? Depending on what we pick, the order on both sides could change, or only on one side. So we should consider the effect of removing an edge from the elements graph on both attribute A and attribute B, which can be very complex.

% % \end{enumerate}

% % I do not currently have an alternative for discovering approximate SOCs when we are dealing with a non-empty context. But if we are only concerned with the second level of the lattice (empty context), we only have to deal with issue number 1 discussed above, and we could compute the coverage of all the chains and stick with the one with the biggest coverage.
% % \end{colorful}

==> backup.tex <==
% SECTION 3.1:

\subsection{Implicit Domain Orders} \label{sec:implicit orders}

%\begin{change}
For \emph{explicit-explicit} \OC\ discovery,
say, for columns \A{A}\ and \A{B},
it suffices to check that the tuples of \T{r}\
can be ordered in \emph{some} way
that is consistent \emph{both}
with ordering the tuples of \T{r}\
with respect to column \A{A}'s explicit domain order
\emph{and}
with respect to column \A{B}'s explicit domain order.
That way of ordering the tuples of \T{r}\
is a \emph{witness} that \A{A}\ and \A{B}\ can be ``co-ordered'';
it \emph{justifies} that \oc{\A{A}}{\A{B}}.

To define \emph{explicit-implicit order compatibility},
we want to maintain this same concept:
there is a way to order the tuples of \T{r}\
with respect to column \A{A}'s explicit domain order
\emph{and} for which the projection on \A{B}\ provides
a \emph{valid} order over \A{B}'s values.
That order on \A{B}\ is valid \emph{iff}
no value of \A{B}\ appears in two different places in the ordered list
with some other value of \A{B}\ in between;
that is, there are no ``cycles''.
This answers one of our two questions:
whether the candidate \OC\ of \oc{\A{A}}{\A{B}[][*]}\ \emph{holds}
over \T{r}.
The second question in this case, though,
that we also need to answer is,
what is \emph{that} order \A{B}[][*]?

% In the next section,
% we shall refine this
% for \emph{implicit-implicit order compatibility}.

Such a witness order over \T{r}\
derives a strong total order over \A{B}.
There may be more than one witness order over \T{r}.
%that suffices.
Consider the $\OC$ $\simular{\A{monthNum}}{\A{monthLun}^*}$ over the first five tuples in Table~\ref{table:festivals}. While the ordering $[\tup{t}_1, \tup{t}_2, \tup{t}_3, \tup{t}_4, \tup{t}_5]$ is a valid witness that gives the order $Corner\prec Peach\prec Plum\prec Pomegranate\prec Winter$ over $\A{monthLun}$, so is the ordering $[\tup{t}_1, \tup{t}_3, \tup{t}_2, \tup{t}_4, \tup{t}_5]$, where the order of month values $Peach$ and $Plum$ is swapped. This indicates that we can only derive a \emph{weak} total order $Corner\prec\{Peach, Plum\}\prec Pomegranate\prec Winter$. 
%however.
% % Previous idea
% Consider when \fd{\A{B}}{\A{A}}.
% Any witness order over \T{r}\
% orders the partition groups over \T{r}\
% with respect to \A{A}.
% This orders the \emph{groups} of \A{B}-values,
% and also dictates the order of \A{B}-values
% within each group.
% A different witness order over \T{r}\
% must order the partition groups over \T{r}\
% with respect to \A{A}\ in the same way,
% of course,
% but orders the \A{B}-values
% within groups differently.
% In composite,
% we know the order of the \A{B}-groups,
% but not the values within each group.
% %
% Overall then,
% the dictated order of \emph{groups} of \A{B}-values,
% \A{B}[][*],
% in this case
% is a \emph{weak} total order over \A{B}.

When we consider an \EIOC\ with a non-empty context,
\oc[\set{X}]{\A{A}}{\A{B}[][*]},
then there must be a witness total order over \T{r}\
that is,
\emph{within} each partition group of \set{X},
compatible with the explicit order of \A{A}\
\emph{and},
\emph{within} each partition group of \set{X},
the order over \A{B}\ dictated by this is valid.
%
This time,
the most that we can derive about \A{B}[][*]\
might not be a weak total order,
but it is a strong partial order.

If \oc[\set{X}]{\A{A}}{\A{B}[][*]}\ holds over \T{r},
what then is the ``strongest'' \A{B}[][*]?
We define it as
the intersection of all the derived strong total orders over \A{B}\
corresponding to the possible witness total orders of \T{r}\
that justify \oc[\set{X}]{\A{A}}{\A{B}[][*]}.
This is a ``model-theoretic'' definition.
Of course,
it would be impractical to find \A{B}[][*]\ this way.
We will present an algorithm, a ``proof-theoretic'' definition,
for discovering \A{B}[][*].

\begin{definition}
(\emph{strongest derived order via an \EIOC})
\label{DEF/EIOC holds and B*}
%
The \EIOC\ of
\oc[\set{X}]{\A{A}}{\A{B}[][*]}\
\emph{holds} over \T{r}\
\emph{iff}
there exists a \emph{witness} strong total order
\Ord{T}[\T{r}][\prec]\
such that,
for \(\tup{s}, \tup{t} \in \T{r}\),
if \(\tup{s} \prec \tup{t} \in \Ord{T}[\T{r}][\prec]\)
and
\(\tup{s}[\set{X}] = \tup{t}[\set{X}]\),
then
\(\tup{s}[\A{A}] \prec \tup{t}[\A{A}] \in \Ord{T}[\A{A}][\prec]\),
and 
the derived ``order'' relation over \A{B},
\[
    \Ord{T}[{\A{B}[][*]}][\prec] =
	\{
		\tup{s}[\A{B}] \prec \tup{t}[\A{B}]
	\,|\,
		\tup{s} \prec \tup{t} \in \Ord{T}[\T{r}][\prec]
			\land
		\tup{s}[\A{B}] \ne \tup{t}[\A{B}]
			\land
        \tup{s}[\set{X}] = \tup{t}[\set{X}]
	\}\mbox{,}
\]
\noindent
is a strong partial order.

Let \oc[\set{X}]{\A{A}}{\A{B}[][*]}\
hold over \T{r},
and \OrdColl{B}\ be the \emph{collection}
of derived order relations over \A{B}\
with respect to the witness orders over \T{r}.
The \emph{strongest derivable} (strong partial) \emph{order}
over \A{B}\
is defined as
\[
	\A{B}[][*]
		=
	\bigcap_{\Ord{T}[\A{B}][\prec]\in\OrdColl{B}} \Ord{T}[\A{B}][\prec]%
	\mbox{.}
\]
\end{definition}

% \begin{definition} \label{def:iioc}
% We call $\simularCtxSet{\set{X}}{\A{A}}{\A{B}^*}$ a valid $\IIOC$
% candidate, iff there exists a strong total order
% \Ord{T}[{\A{B}[][*]}][\prec] s.t. when applying over the values of
% $\A{B}$, no \emph{swap}s exists between any two tuples in the
% dataset.
% \end{definition}

% While $\EIOD$s are defined in a similar fashion. Our goal in this
% section is to not only verify a given $\IIOC$ candidate
% $\simularCtxSet{\set{X}}{\A{A}}{\A{B}^*}$, but to also determine a
% strong partial order \Ord{P}[{\A{B}[][*]}][\prec] $\subseteq$
% \Ord{T}[{\A{B}[][*]}][\prec], where the order relations in
% \Ord{P}[{\A{B}[][*]}][\prec] are supported by some \emph{evidence}
% in the dataset.

% \vspace{-1mm}
\begin{example}
The \EIOC\ of \oc{\A{yearLun}}{\A{monthLun}[][*]}\
holds over the first five tuples
in Table~\ref{table:festivals}.
There is a single value for 
%the attribute 
\A{yearLun}.
That there exists a total order
over the tuples with no cycle
over the values of \A{monthLun}\ (``\A{B}'')
means then that there is a valid witness.
% over the values of \A{monthGreg}\ does not cause
% swaps in the table.
%Thus,
%\oc{\A{yearLun}}{\A{monthLun}[][*]}\ holds
%over the first five tuples of Table~\ref{table:festivals}.
%In this case,
However,
since \emph{all} such total orders not causing a cycle
(all of them in this case),
we have no information regarding
the order between month values,
besides that they can be arbitrarily ordered here.
Thus,
\(\A{monthLun}[][*] = \emptySet\),
the \emph{empty} partial order.
\end{example}

% =======================================================================================







